Industrial scale large eddy simulations (LES) with adaptive octree meshes using immersogeometric analysis

We present a variant of the immersed boundary method integrated with octree meshes for highly efficient and accurate Large-Eddy Simulations (LES) of flows around complex geometries. We demonstrate the scalability of the proposed method up to $\mathcal{O}(32K)$ processors. This is achieved by (a) rapid in-out tests; (b) adaptive quadrature for an accurate evaluation of forces; (c) tensorized evaluation during matrix assembly. We showcase this method on two non-trivial applications: accurately computing the drag coefficient of a sphere across Reynolds numbers $1-10^6$ encompassing the drag crisis regime; simulating flow features across a semi-truck for investigating the effect of platooning on efficiency.

==> Data/WeightedPartitionPlot.tex <==
\begin{figure*}[t!]
\begin{tikzpicture}
  \begin{groupplot}[
      group style={group size=2 by 1,ylabels at=edge left,vertical sep=50pt},
      ylabel style={text height=0.02\textwidth,inner ysep=0pt},
      xlabel= Relative weight of \Intercepted elements, % Set the labels
      ylabel= Time (in s),
      log ticks with fixed point,
      height=0.3\linewidth,width=0.5\linewidth,/tikz/font=\small
    ]
    \nextgroupplot[xmode=log,log basis x={10},title={\textbf{Matrix Assembly}}]%
     \addplot
         table[x expr={0.001*\thisrow{Weight}))},y expr=\thisrow{MatVol},col sep=space]{Data/WeightedPartition.txt};
        \addplot
        table[x expr={0.001*\thisrow{Weight}))},y expr=\thisrow{MatSurf},col sep=space]{Data/WeightedPartition.txt};
        \addplot
         table[x expr={0.001*\thisrow{Weight}))},y expr=\thisrow{MatTotal},col sep=space]{Data/WeightedPartition.txt};
    \coordinate (bot) at (rel axis cs:1,0);% coordinate at bottom of the last plot
    
    \nextgroupplot[xmode=log,log basis x={10},title={\textbf{Vector Assembly}}]%
    \addplot
         table[x expr={0.001*\thisrow{Weight}))},y expr=\thisrow{VecVol},col sep=space]{Data/WeightedPartition.txt};
         \label{plot:volume}
        \addplot
        table[x expr={0.001*\thisrow{Weight}))},y expr=\thisrow{VecSurf},col sep=space]{Data/WeightedPartition.txt};
        \label{plot:surf}
        \addplot
         table[x expr={0.001*\thisrow{Weight}))},y expr=\thisrow{VecTotal},col sep=space]{Data/WeightedPartition.txt};
         \label{plot:total}
    \coordinate (top) at (rel axis cs:0,1);% coordinate at top of the first plot
     
  \end{groupplot}
  % legend
  \path (top|-current bounding box.south)--
        coordinate(legendpos)
        (bot|-current bounding box.south);
  \matrix[
      matrix of nodes,
      anchor=north,
      draw,
      inner sep=0.2em,
    ]at([yshift=-1ex]legendpos)
    { \ref{plot:volume}& Volume cost &[5pt]
      \ref{plot:surf}& Surface cost &[5pt]
      \ref{plot:total}& Total cost &[5pt]\\};
\end{tikzpicture}
\caption{Effect of weighted partitioning on the matrix and vector assembly time. The cost of volumetric assembly increases with increase in the relative weight of the \Intercepted nodes and the surface assembly decreases.}
\label{fig:Wpart}
\end{figure*}

\begin{figure}[t!]
\begin{tikzpicture}
      \begin{loglogaxis}[
          width=0.85\linewidth, % Scale the plot to \linewidth
          %grid=major, % Display a grid
          %grid style={line width=.1pt, draw=gray!50}, % Set the style
          xlabel=Relative weight of \Intercepted elements, % Set the labels
          ylabel=Time (in s),
          ymax = 500,
          log ticks with fixed point,
          legend style={legend columns=1}, % Put the legend below the plot
          x tick label style={rotate=0,anchor=north} % Display labels sideways
        ]
        \addplot 
        table[x expr={0.001*\thisrow{Weight}))},y expr=\thisrow{Solve},col sep=space]{Data/WeightedPartition.txt};

        \addplot 
        table[x expr={0.001*\thisrow{Weight}))},y expr=\thisrow{MatTotal},col sep=space]{Data/WeightedPartition.txt};
        
        % \addplot 
        % table[x expr={0.001*\thisrow{Weight}))},y expr=\thisrow{VecVol},col sep=space]{Data/WeightedPartition.txt};
        % \addplot 
        % table[x expr={0.001*\thisrow{Weight}))},y expr=\thisrow{VecSurf},col sep=space]{Data/WeightedPartition.txt};
        \addplot 
        table[x expr={0.001*\thisrow{Weight}))},y expr=\thisrow{VecTotal},col sep=space]{Data/WeightedPartition.txt};
        
        
         \legend{\small{Total solve time},\small {Matrix Assembly},\small {Vector Assembly}}
        \end{loglogaxis}
        \end{tikzpicture}
        \caption{Effect of weighted partitioning on the matrix assembly, vector assembly and total solve time. }
          \label{fig: WPartAssembly}
\end{figure}


==> Plots/TruckFrontPage.tex <==
\begin{figure*}[t!]
  \includegraphics[width=1.0\linewidth]{Figures/Truck/FrontPageFig/FrontPage_onetruck-with-backgorund.png}
  \caption{Render image of flow passing a semi-trailer truck.}
%   \caption{Render image of flow passing two semi-trailer trucks.}
  \label{fig: TruckFrontPage}
\end{figure*}


==> Plots/TruckLICmidzplane.tex <==
\begin{figure}[t!]
  \centering
  \includegraphics[width=0.8\linewidth]{Figures/Truck/LIC_mid_z.png}
  \caption{Flow structure at vertical middle plane.}
  \label{fig: TruckLICmidz}
\end{figure}

==> Plots/TruckLICxplane.tex <==
\begin{figure}[t!]
  \centering
  \includegraphics[width=1.0\linewidth]{Figures/Truck/LIC_slices_in_x.png}
  \caption{Flow structure slices in $x$ direction.}
  \label{fig: TruckLICx}
\end{figure}

==> ad.tex <==
% artifact description goes here. 
\appendix
\subsection{Artifact Availability}
\subsubsection{Software Artifact Availability}

The \IMGAcode~ simulation code is freely available at Bitbucket  (link will be disclosed after review process) under the GNU General Public License (GPL). 
The latest version of the code can be obtained by cloning the repository
\begin{lstlisting}[language=bash,basicstyle=\small]
$ git clone https://bitbucket.com/IMGA/XXX.git
\end{lstlisting}
The following dependencies are required to compile \IMGAcode~
\begin{itemize}
	\item C/C++ compilers with C++11 standards and OpenMP support
	\item MPI implementation (e.g. openmpi, mvapich2 )
	\item Petsc 3.7 or higher
	\item ZLib compression library (used to write \texttt{.vtu} files in binary format with compression enabled)
	\item  LAPACK or MKL are only needed, if  doing the tensor operations
	\item CMake 2.8 or higher version
	\item \href{http://hyperrealm.github.io/libconfig}{libconfig} for parameter reading from file.
\end{itemize}
After configuring \IMGAcode, generate the Makefile (use \texttt{c} to configure and \texttt{g} to generate). Then execute \texttt{make all} to build all the targets.
Please follow the instruction page on the repository for more details on installation.

\subsection{Experiments}
All the experiments reported using \Stampede~ are executed in the following module environment. 
\begin{verbatim}
Currently loaded modules :
1) intel/17.0.4     2) impi/17.0.3 
3) cmake/3.16.1     4) git/2.9.0
5) autotools/1.1    6) petsc/3.7 
\end{verbatim}

Experiments performed in \Frontera~ are executed in the following module environment. 
\begin{verbatim}
Currently Loaded Modulefiles:
  1) intel/19.0.5   4) python3/3.7.0
  2) impi/19.0.5    5) autotools/1.2
  3) petsc/3.12     6) cmake/3.16.1
\end{verbatim}

Additionally, on \Frontera~ we set  the following environment variables:
\begin{verbatim}
    export I_MPI_ADJUST_ALLREDUCE=1
\end{verbatim}

\subsubsection{Matrix Assembly}
The code must be compiled with option \textsc{DTENSOR=Yes} during the compile time which will enable the matrix - matrix multiplication based assembly describes in \ref{sec: MatrixAssembly}. The config file is provided under the repository folder \texttt{tests/MatrixAssembly}. The element order from linear to quadratic can be changed by changing the \texttt{BasisFunction} in the config file.

\subsubsection{Weighted partition}
The Weighted partition tests can be performed under the repository folder {tests/WeightedPartitioning}. \added{The ratio of volume to the surface  cost can be changed for variable \texttt{RatioWeight} in the config file.}

\subsubsection{Adaptive quadrature}
The Weighted partition tests can be performed under the repository folder \texttt{tests/AdaptiveQuadrature}. The maximum level of split can be changed by changing the parameter \texttt{gp\_max\_splitting}. The adaptive quadrature is only activated when \texttt{gp\_handle} is set to 32.

\subsubsection{Scaling}
The config file for scaling tests are provided  under the repository folder {tests/Scaling}. The detailed instruction to create all 4 different meshes are provided in the folder.

In order to run the cases, please use:
\begin{verbatim}
    ibrun -np <mpi tasks> 
    ./${PATH_TO_EXECUTABLE} -log_view
\end{verbatim}
\subsection{\Stampede~ SKX compute node configuration}

\begin{verbatim}
    TACC_SYSTEM=stampede2
    Architecture:          x86_64
    CPU op-mode(s):        32-bit, 64-bit
    CPU(s):                96
    Thread(s) per core:    2
    Core(s) per socket:    24
    Socket(s):             2
    NUMA node(s):          2
    Vendor ID:             GenuineIntel
    CPU family:            6
    Model:                 85
    Model name:            Intel(R) Xeon
                           Platinum 8160 
                           CPU @ 2.10GHz
    CPU MHz:               2100.000
    L1d cache:             32K
    L1i cache:             32K
    L2 cache:              1024K
    L3 cache:              33792K
    
    MemTotal:       196438176 kB
    MemFree:        191589692 kB
    MemAvailable:   190917852 kB
\end{verbatim}

\subsection{\Stampede~ KNL compute node configuration}
\begin{verbatim}
    Architecture:          x86_64
    CPU op-mode(s):        32-bit, 64-bit
    Byte Order:            Little Endian
    CPU(s):                272
    On-line CPU(s) list:   0-271
    Thread(s) per core:    4
    Core(s) per socket:    68
    Socket(s):             1
    NUMA node(s):          1
    Vendor ID:             GenuineIntel
    CPU family:            6
    Model:                 87
    Model name:            Intel(R) Xeon
                           Phi(TM) 7250
                           CPU @ 1.40GHz
    Stepping:              1
    CPU MHz:               1358.813
    CPU max MHz:           1600.0000
    CPU min MHz:           1000.0000
    BogoMIPS:              2793.77
    L1d cache:             32K
    L1i cache:             32K
    L2 cache:              1024K
    
    MemTotal:       98698220 kB
    MemFree:        91011748 kB
    MemAvailable:   90450128 kB

\end{verbatim}
\vfill
\pagebreak

\subsection{\Frontera~ compute node configuration}
\begin{verbatim}
    Architecture:          x86_64
    CPU op-mode(s):        32-bit, 64-bit
    Byte Order:            Little Endian
    CPU(s):                56
    On-line CPU(s) list:   0-55
    Thread(s) per core:    1
    Core(s) per socket:    28
    Socket(s):             2
    NUMA node(s):          2
    Vendor ID:             GenuineIntel
    CPU family:            6
    Model:                 85
    Model name:            Intel(R) Xeon
                           Platinum 8280
                           CPU @ 2.70GHz
    Stepping:              7
    CPU MHz:               2700.000
    BogoMIPS:              5400.00
    Virtualization:        VT-x
    L1d cache:             32K
    L1i cache:             32K
    L2 cache:              1024K
    L3 cache:              39424K
    
    MemTotal:       195920208 kB
    MemFree:        168962328 kB
    MemAvailable:   168337408 kB
\end{verbatim}
\vfill
